Development of a Capacitance Measurement for Pulsed Magnetic Fields

Capacitance measurements are crucial for probing the electrical properties of materials. In this study, we develop and implement a capacitance measurement technique optimized for pulsed magnetic fields. Our approach employs an auto-balancing bridge method, leveraging a high-bandwidth transimpedance amplifier to mitigate parasitic contributions from coaxial cables. This technique enables precise capacitance measurements in rapidly changing magnetic fields, as demonstrated in experiments on the magnetoelectric material NiCo$_{2}$TeO$_{6}$. The results reveal strong magnetoelectric coupling, including a pronounced hysteresis in capacitance that coincides with magnetization measurements and an enhanced energy dissipation peak at high sweep rates. Compared to traditional LCR meter measurements in DC fields, our method exhibits excellent agreement while providing additional insight into field-induced phase transitions. This work establishes a robust methodology for capacitance measurements in extreme conditions and opens new opportunities for studying multiferroic and correlated electron systems under high magnetic fields.

==> authorinfo.tex <==
William K. Peria
Shengzhi Zhang
Sangyun Lee
Vivien Zapf
Choongjae Won
Sang-Wook Cheong
Minseong Lee

email: 
william.peria@nist.gov
shengzhi@lanl.gov
sangyun.lee@ufl.edu
vzapf@lanl.gov
cjwon@mpk.or.kr
sangc@physics.rutgers.edu
ml10k@lanl.gov
